Tight Lower Bound on Equivalence Testing in Conditional Sampling Model

We study the equivalence testing problem where the goal is to determine if the given two unknown distributions on $[n]$ are equal or $\epsilon$-far in the total variation distance in the conditional sampling model (CFGM, SICOMP16; CRS, SICOMP15) wherein a tester can get a sample from the distribution conditioned on any subset. Equivalence testing is a central problem in distribution testing, and there has been a plethora of work on this topic in various sampling models. Despite significant efforts over the years, there remains a gap in the current best-known upper bound of $\tilde{O}(\log \log n)$ [FJOPS, COLT 2015] and lower bound of $\Omega(\sqrt{\log \log n})$[ACK, RANDOM 2015, Theory of Computing 2018]. Closing this gap has been repeatedly posed as an open problem (listed as problems 66 and 87 at sublinear.info). In this paper, we completely resolve the query complexity of this problem by showing a lower bound of $\tilde{\Omega}(\log \log n)$. For that purpose, we develop a novel and generic proof technique that enables us to break the $\sqrt{\log \log n}$ barrier, not only for the equivalence testing problem but also for other distribution testing problems, such as uniblock property.

==> LB.tex <==


\section{$\Tilde{\Omega}(\log \log n)$ lower bound for Equivalence testing}







\subsection*{Construction of hard instances}
\label{sec:hardinstance}
%We will set the value of parameters $\phi,\rho,\alpha$ later. 
We give a randomized procedure to generate an input for equivalence testing.  %First, we randomly chose between YES and NO prior (i.e., we select YES with probability $1/2$ and NO with probability $1/2$). %
We will construct two priors $YES$ and $NO$ over a pair of distributions on $[n]$. 
For the NO instance,  we randomly generate   a pair of distributions by the following procedure:
\begin{enumerate}
    \item A  number $x \in \{0,1,\dots,\frac{\log n}{2}\}$ is chosen uniformly at random. We have $b=2^{x}$ and let $m = b(\rho++\rho^2+\dots,\rho^r)$.
    \item A pair of distribution $(Q_1,Q_2)$ is constructed as follows: We randomly choose a subset of size $m$ from $[n]$ that forms the support of both distributions $Q_1$ and $Q_2$. We then randomly partition the supports into $r$ buckets (for both $Q_1$ and $Q_2$) $B_1,\dots,B_r$ such that $|B_j| = b \rho^j$ and assign the probability $1/r$ to each bucket. In distribution $Q_1$, the probability distribution is uniform in each bucket, i.e., for all $j \in [r],$ we have  $Q_1(i) = \frac{1}{r b \rho^j}$ for each $i \in B_j$. In distribution $Q_2$, each bucket $B_j$ is randomly partitioned into two subbuckets $B^e_j$ and  $B^w_j$ of equal size ($ = \frac{|B_j|}{2}$) such that $Q_2(B^e_j) = \frac{3}{4r}$ and $Q_2(B^w_j) = \frac{1}{4r}$ and distribution is uniform in each subbuckets. In other words, we have $Q_2(i) = \frac{3}{2rb \rho^j}$ for $i \in B^e_j$ and $Q_2(i) = \frac{1}{2rb \rho^j}$ for $i \in B^w_j$, for all $j \in [r]$.
    \item The pair of distribution $(Q_1,Q_2)$ is returned.
\end{enumerate}
For the YES case, the procedure to generate a pair of distributions is the same as that of NO except  that pair $(Q_1,Q_1)$ is returned (instead of $(Q_1,Q_2)$). We set  $\rho = 2^{\sqrt{\log n}}$  and $r = \frac{\sqrt{\log n}}{4}$. %Let $ \{0,1,\dots,\frac{\log n}{2}\}$. 
%$\alpha = (\log n)^{(\log \log n)^4}$
%For any $k_b \in  \{0,1,\dots,\frac{\log n}{2}\}$, let $b = 2^{k_b}$. We will now generate two distributions $D_1$ and $D_2$ randomly.

%Fix  $k_b \in \{0,1,\dots,\frac{\log n}{2}\}$ uniformly at random. The distribution $D_1$ can be divided into $r$ buckets $B_1,B_2,\dots,B_r$ such that $|B_j| = b \rho^j$ for all $j \in [r]$. Further, the probability mass of each bucket is equal, i.e., $\frac{1}{r}$. Therefore, probability of any element in bucket $j$ is $\frac{1}{rb\rho^j}$ for all $j \in [r]$. Note that the support of the distribution is $b \sum_{j \in [r]}\rho^j = b \rho \frac{\rho^r - 1}{\rho -1 } = b \Theta(n^{1/4})$.

%The distribution $D_2$  has same support as that of $D_1$. It can also be divided into $r$ buckets $B_1,B_2,\dots,B_r$ such that $|B_j| = b \rho^j$ for all $j \in [r]$. Here also, the probability mass of each bucket is $\frac{1}{r}$. However, the probability mass of each  element in a fixed bucket are not equal. Let for each $j \in [r]$,  $B_j = B^e_j \cup B^w_j$ be a random partition of bucket $j$ such that $|B^e_j| = |B^w_j| = \frac{|B_j|}{2}$. The probability of any element in $B^e_j$ is $\frac{3}{2rb \rho^j}$ and any element in $B^w_j$ is $\frac{1}{2rb \rho^j}$.
Note that the total variation distance between distributions $D_1$ and $D_2$ is $\frac{1}{2} \sum_{i \in [r]} \frac{1}{2rb \rho^j} \cdot b \rho^j = \frac{1}{4}$. 
%The yes instance for the equivalence testing problem is $(D_1,D_1)$ and for no instance is $(D_1,D_2)$. We will prove the following theorem later.
%In section~\ref{sec:lbsupport}, we will prove the following theorem.
%\begin{theorem}
%\label{thm:lower-support}
%Suppose $k_b$ is chosen at random and we are given COND access to the distribution $D_1$.  Any tester that  makes $q$ queries to determine $k_b$ will have a probability of error at least $1 - \frac{q \log \log \log n}{\log \log n}$. 
%\end{theorem}


\subsection*{Proof Sketch}
%\paragraph*{On the application of Yao's theorem:}
By Yao's theorem, to show our main theorem, it suffices to show the lower bound for any deterministic counterpart of  core adaptive  tester (say $T$) for random instances described in section. We want to point out that even though $D$ will have no internal randomness (no coin toss by the tester) but it will continue to have external randomness (i.e., randomness in the outcome of $COND$ oracle).% For this reason, we will refer to it as the deterministic counterpart of the core adaptive tester.

The tester $T$, for any $i \le q$,  maps a sequence of configurations $(c_1,\dots,c_{i-1})$ of the received samples so far, via a deterministic function $f_T$, to a pair  $(O_i, U_i)$ (where $O_i \subseteq  \{s_1,\dots,s_{i-1}\}$ and $U_i \subseteq [n]\setminus \{s_1,\dots,s_{i-1}\}$) which determines the $i$th query set is $A_i = O_i \cup U_i$.

%From the previous configurations $(c_1,\dots,c_{i-1})$ (with respect to previous query-sample pairs $((A_1,s_1),\dots,(A_{i-1},s_{i-1}))$), the tester $T$  deterministically determines 
%$k^A_i$ for each atom $A \in At(A_1,\dots,A_{i-1})$ and $K_i \subseteq [i-1]$ say via a function $f_T$. %Thus the tester $T$ can be fully described by the first query set $A_1$ and a deterministic function $f_T$ that maps $(c_1,\dots,c_{i-1})$ to a pair $(O_i,U_i)$ (where $O_i \subseteq  \{s_1,\dots,s_{i-1}\}$ and $U_i \subseteq [n]\setminus \{s_1,\dots,s_{i-1}\}$) such that the $i$th query set is $A_i = O_i \cup U_i$.



%In a natural way, the tester $T$ can also be fully described by a decision tree $R$ where the path (from root) to any node $v$ at depth $i$ (more precisely, the edges of this path) corresponds to the configuration of the first $i-1$ samples. Note that fixing the configurations of the samples till $i-1$ queries (and the internal randomness) fixes the size of an atom $A \in At(A_1,\cdots,A_i)$ (and hence of each $A_j$ for $j \le i$). %However, the sets $A_1,\cdots,A_i$ themselves are not fixed and are random variables (as the counter constructs such sets using its internal randomness). 
In a natural way, the tester $T$ can also be fully described by a decision tree $R$. Formally, the edges of a path (from root) to any node $v$ at depth $i$ is associated with a sequence of configurations $(c_1,\dots,c_i)$ and the node $v$ is labeled with a pair $(O_v, U_v) = f_T(c_1,\dots,c_i)$ (where $O_v \subseteq \{s_1,\dots,s_i\}$ and $U_v \subseteq [n] \setminus \{s_1,\dots,s_i\}$)   which determines the next query set $A_{v} = O_v \cup U_v$.
    Further, for every possible value of the configuration $c_{i+1}$ of the sample from $A_{v}$, there is a corresponding child of the node $v$ and the corresponding edge is labeled by the value of configuration $c_{i+1}$. 

%Given a sequence of  pairs $((A_1,C_1),\dots,(A_{i-1},C_{i-1}))$ (where for $j \le i-1$,  $A_j$ is the $j$th query set and $C_j$ is the configuration of the sample from $A_j$),  the next query set $A_i = O_i \cup U_i$ by the tester is uniquely determined in any deterministic counterpart of the core adaptive tester. Formally, any such tester $T$ can be fully specified by  the first query set $A_1$ and a deterministic function $f_T$ that maps a sequence of  pairs $((A_1,C_1),\dots,(A_{i-1},C_{i-1}))$ to a pair $(O_{i},U_{i})$\footnote{(the sets $O_{i+1}$ and $,U_{i+1}$ are subset of seen and unseen elements respectively, as defined in the definition of core adaptive tester} which determines the $i$th query set $A_i = O_i \cup U_i$.

%and a sequence of configurations of obtained samples $s_1,\dots,s_{i-1}$ from $A_1,\dots,A_{i-1}$ respectively, the next query set $A_i = O_i \cup U_i$ by the tester is uniquely determined in any deterministic counterpart of the core adaptive tester. % A \emph{transcript} of the tester after $i$-queries denoted by $\tau(i)$ (for some $i \le q$) consists of a  sequence of query sets $(A_1,\dots,A_{i})$ by the tester and a sequence of configurations $C_1,\dots,C_{i}$ of the obtained samples.
%Formally, any deterministic tester $T$ can be fully specified by  the first query set $A_1$ and a deterministic function $f_T$ that maps a sequence of query sets  $(A_1,\dots,A_{i})$ and configurations of the samples to a pair of sets $(O_{i+1},U_{i+1})$(the sets $O_{i+1}$ and $,U_{i+1}$ are subset of seen and unseen elements respectively, as defined in the definition of core adaptive tester) such that $A_{i+1} = O_{i+1} \cup U_{i+1}$ is the $(i+1)$th query set. 
%The state of the tester  after $i$ queries is a tuple $((A_1,C_1),(A_2,C_2),\dots,(A_i,C_i),A_{i+1})$ where 

%$((A_1,\dots,A_{i-1}), (C $

%consists of first $i$ queries, the configuration of the obtained samples and the $(i+1)$th query set determined by $f_T$. Note that for any $i \le q$, transcript $\tau(i)$ and $\mcS(i)$ are random variables, i.e., a different \emph{run} of the tester (on same input) may have different transcript and state.


%In a natural way, a $q$-query deterministic tester $T$ given by $A_1$ and $f_T$ can be specified by a decision tree $R_T$ of depth $q$. The root of $R_T$ is labeled by the query set $A_1$. In general, any node $v$ is labeled by a query set $A_v = O_v \cup U_v$ and an edge is labelled by a configuration. A path to $v$ at depth $i$ (from root) corresponds (in one to one manner) to a sequence of pairs $((A_1,C_1),\dots,(A_{i},C_{i}))$ such that $A_1,\dots,A_{i}$ are the labels of the nodes in the path (in order) and $C_1,\dots,C_{i-1}$ are the labels of the edges in this  path (in order). Further, we have $(O_v,U_v) = f_T(((A_1,C_1),\dots,(A_{i-1},C_{i-1}))$. A run of a tester corresponds to a path taken by the tester (from the root  to a leaf). Note that  $|R_T|$, i.e., the number of nodes in $R_T$ is at most $2^{q^2}$.

We now define notations that we will use throughout the paper.  We will use $(O_v,U_v)$ for the label of a node $v$ and $A_v = O_v \cup U_v$ for the corresponding query set. Let the nodes of the path from root to the node $v$ be $v_0,v_1,\dots,v_i$ where $v_0$ is the root and $v_i$ is the node $v$. We will use  $\bm{A}_v = (A_{v_0},\dots,A_{v_i})$ for the sequence of the query sets corresponding to the  nodes in this path. Further, $At(\bm{A}_v) := At(A_{v_0},\dots,A_{v_i})$. Note that the set of all relevant atoms for the tester is  $\cup_{v \in R} At(\bm{A}_v) $ which will be denoted by $At(R)$.

%The set of all possible atoms in $R$, i.e., $\cup_{v \in R} At(\bm{A}_v) = \cup_{v \in R} At((A_1,\dots,A_v))$ is denoted by $At(R)$. 

%In general, a path $()$ to $v$ (from root) corresponds (in one to one manner) to a sequence of pairs $((A_1,C_1),\dots,(A_{i-1},C_{i-1}))$ w


%In the decision tree $R_T$, any node $v$ (at depth $i$) is labeled by a query set $A_v = O_v \cup U_v$ (and the root is labeled by $A_1$) and a path to $v$ (from root) corresponds (in one to one manner) to a sequence of pairs $((A_1,C_1),\dots,(A_{i-1},C_{i-1}))$ such that query set $A_j$ is the label of the $j$th node in this path,  configuration of  


 



%every possible state of the tester after $i$-queries corresponds to a node at depth $i$, in one to one manner.  Formally,  any node $u$ is associated with the tuple $(O_u, U_u, A_u)$ where $A_u = O_u \cup U_u$ and when $u$ is the root, the associated tuple is $(\emptyset,A_1,A_1)$.  For every possible value of configuration of sample from $A_u$, there is a corresponding child $v$ of $u$ such that the edge $(u,v)$ is labeled by the value of configuration. % A path from root to node $u$ corresponds to a state
%A run of a tester corresponds to a path taken by the tester (from the root  to a leaf).
%, an edge $(u,v)$ from node $u$ at depth $i$ to a node $v$ at depth $(i+1)$ is labeled by a possible value of configuration of the obtained sample from $A_u$, a path from root to a node $u$ at depth $i$ corresponds to a state of the tester $\mcS(i)$.

%a path from root (which corresponds to set $A_1$) to a node at depth $i$ corresponds to a transcript of length $i-1$ and vice versa, nodes at depth $i$ correspond to a query set $A_i= O_i \cup U_i$, each edges $(u,v)$ are labeled by the each possible value of configuration of sample $s_i$ from $A_i$.


%In this path,  the edges corresponds to the configuration of the samples,  Further, Sincconfiguration of any sample can take at most $2^q$ values, the size of $R$ is upper bounded by $2^{q^2}$.


%The root of the tree is the first set $A_1$ and  has children corresponding to each possible value of configuration of sample $s_1$ obtained from $A_1$.   In general, any node $u$ is associated with a query set $A_u$ and an edge $(u,v)$ from node $u$ to some node $v$ is labellied by the configuration of the sample $s_u$ obtained from $A_u$ given the sequence of query sets $A_1,f(A_1,c_1),$ Any path from a node to a node at depth $i$ corresponds t
%A node $u$ is associated with a query set $A$ and has children corresponding to each possible configuration of sample $s$ obtained from $A$, edge $(u,v)$ in this tree is labelled by the configuration of the 


%A node $u$ at depth $i$ corresponds, in one to one way, to $i$th query set $A$
%However, the external randomness in the conditional samples from the input distribution will exists and in that sense the algorithm is still randomized.

Our goal is to show the following theorem which (by Yao's min max theorem) will apply our main theorem..

%it suffices to show a lower bound for any (core adaptive) tester in which  tester's internal coin tosses and coin tosses at step 2(i) (of the core adaptive tester) are fixed. 


\begin{theorem}
    \label{thm:equivalence-lb}
    Any deterministic core adaptive tester that, given $COND$-access to a pair of distributions  randomly generated as described in section,  correctly classify the instance as YES or NO, with probability at least $2/3$, must make  $\Tilde{\Omega}(\log \log n)$ $COND$-queries.
\end{theorem}

% Fixing the internal randomness (and randomness at step 2(a)) fixes the nodes of the decision tree $R$. % represents all possible  runs of the tester $T$. 

%Any such deterministic tester $T$ can be fully specified  by its decision tree $R$ (i.e., $R$ does not depend on input distribution) in a natural way. Any path $(u_0,u_1,\dots,u_i)$ from root to a node $u_i$ at depth $i$  corresponds to a sequence of query sets $(A_1,\dots,A_{i-1})$ and $(i-1)$-configuration of the samples $(s_1,\dots,s_{i-1})$ obtained from the respective query sets. More precisely, each node $u_j$ is associated with the query set $A_{u_j}$ and each edge $(u_j,u_{j+1)$ is associated with the the label invariant information that $s_j$ has about

%an $i-1$-configuration (and equivalently, any $(i-1)$-configuration corresponds to a unique node at depth $i$) in a natural way. Thus, total number of nodes at depth $i$ is the cardinality of all possible $(i-1)$-configurations of the tester. More precisely, if $(u_0,u_1,\dots,u_i)$ is an path from the root $u_0$ to a node $u_i$ (at depth $i$) then it corresponds to an $i$-configuration say $(A_1,\dots,A_{i-1})$ and $(s_1,\dots,s_{i-1})$ such that 

%The height of $R$ is $q$. 
%Any internal $u$ node at depth $i$ is associated with a $i$th query set $A_i = O_i \cup U_i$ (for a run corresponding to the path from root to this node)(a path from root to this node specifies the sequence of query sets $(A_1,\dots,A_{i-1})$ and configurations of the samples $(s_1,\dots,s_{i-1})$) and   $j \in \{1,2\}$ (set $A_i$ will be queried on distribution $D_j$).  For each possible outcomes of $s_i$ (obtained from $COND_{D_j}(O_i \cup U_i)$), there is a corresponding child  $v$ of node $u$ such that edge $(u,v)$ is labeled by that outcome. We will denote $O_i$ and $U_i$ associated with any node $u$ at depth $i$ as $O^u$ and $U^u$ respectively. 
 
 %A path from root to any internal $u$ node at depth $i$ is associated with an $(i-1)$-configuration, $j \in \{1,2\}$ and parameters $K_i \subseteq \{1,\dots,i-1\}$ and $k^A_i$ (for each atom $A \in At(A_1,\dots,A_{i-1})$) which specifies the $i$th query set $O_i \cup U_i$ on distribution $D_j$. 


%Note that there are at most $O(q 2^{q^2})$ nodes in $R$ and hence total number of sets $O^u$ and $U^u$ (for each $u$ in $R$) is also upper bounded by  $O(q 2^{q^2})$. We now introduce some notations.

%Fix $x$ and  the distribution $D_x$.
Given as input a pair of distributions $(D_1,D_2)$ (as an oracle), the tester can invoke a conditional sampling oracle for either of the distribution $D_1$ and $D_2$. For $j\in \{1,2\}$, we will denote $COND_j(A)$ as the conditional sampling query on set $A$ in distribution $D_j$. %Note that $COND_j(A)$ also represents a distribution on elements of $A$ where an element $s \in A$ is picked with probability $\frac{D_j(s)}{D_j(A)}$ (if $D_j(A) \neq 0$) or with probability $\frac{1}{|A|}$ (if $D_j(A) = 0$). 
Note that, the possible values of set $A$ is restricted  to the set $\{A_v\}_{v \in R}$ (where $A_v = O_v \cup U_v$). 
Also recall as per our convention, a conditional sampling query $COND_j(O_v \cup U_v)$ 
\begin{enumerate}
    \item first picks an element $e \in O_v \cup \{U_v\}$ (elements of $O_v$ and the set $\{U_v\}$ itself) with probability $\frac{D_j(e)}{D_j(O_v \cup U_v)}$. If $e \in O_v$ then sample $s_i$ is set to $e$. If $e = \{U_v\}$ then
    \begin{enumerate}
        \item An atom $V \in At(U_i)$ is picked with probability $\frac{D_j(V)}{D_j(U_i)}$.
        \item The sample $s_i$ is generated by the $COND_j(V)$. 
    \end{enumerate}
\end{enumerate}


%consists of two steps --- in the first step an element $e$ in $O_i \cup \{U_i\}$ is picked with the probability $\frac{D_j(e)}{D_j(O_i \cup U_i)}$ and if $e = \{U_i\}$ then in second step (i) an atom $V$ in $At(U_i)$ is picked with probability $\frac{D_j(V)}{D_j(U_i)}$ and (ii) a sample $s \in V$ is drawn with probability $\frac{D_j(s)}{D_j(V)}$.

The main analytic difficulty is to understand the probability $\frac{D_j(V)}{D_j(U_i)}$. Note that even though $\frac{\E[D_j(V)]}{\E[D_j(U_i)]} = \frac{|V|}{|U_i|}$, it is not possible to guarantee tight concentration bounds for every $S \in At(R)$, because the size of the decision tree $R$ is large ($2^{q^2}$). Previous approaches tries to bound the number of queries $q$ for which for which tight concentration bounds can be shown for all $S \in At(R)$. This threshold in both works comes out to be $O(\sqrt{\log \log n})$.  Now since for any atom $V$,  we have $D_j(V) \approx \E[D_j(V)]$ (for all $j \in \{1,2\}$) (and by our choice of input distributions, $\E[D_1(V)] = \E[D_2(V)]$ for all $V$), the distributions induced on the leaves of the decision tree, for both YES and NO instances, are statistically close and hence the tester can not classify the instance correctly by making $q < \sqrt{\log \log n})$ queries.

We follow a different approach and do not restrict $q$. We show that even though, a small proportion but a large number of nodes may not have a concentration (we call them bad nodes), the tester will pass through such nodes with a small probability. At a higher level, previous work does not consider the tester's distribution over paths in $R$, rather they find the threshold value of $q$ for which all nodes will have a concentration (which will trivially prove tester will not pass through bad nodes). We, on the other hand, show that even though a small proportion but a large number of nodes can be bad  but the tester, will behave random (we mean randomness independent of the input distribution) for many choices and thus with a high probability, will avoid these nodes. For the same, we study the behavior of the tester when instead of conditional sampling oracle, samples are provided to the tester from a different and simpler oracle called Ratio oracle. This oracle is the same as that of conditional sampling oracle except for an atom $V \in At(U_i)$ is now picked with probability $\frac{|V|}{|U_i|}$ (instead of $\frac{D_j(V)}{D_j(U_i)}$). Surprisingly, the study of the tester's behavior in this oracle leads us to show our desired property (the the tester will not pass through bad nodes) for the original tester also.
%try to show tight concentration bounds for $D_j(S)$ for all relevant set $S$ which can be $2^{O(q^2)}$. When  $q = o(\sqrt{\log \log n})$ we have $2^{O(q^2)} = o(\log n)$. In this case, by union bound, they are able to show tight concentration bounds for all query sets/atoms in $R$. However, this is not tight analysis --- as it is possible that  

% Since all nodes corresponding to the decision tree $R$ 

%For any node $u$, the distribution $COND_j(A_u)$ picks an element $e$ in $O_i \cup \{U_i\}$ with probability $D_j(e)/D(A_u)$, and if $e = \{U_i\}$ then it picks an atom $V$ in $At(U_i)$ with probability $D_j(V)/D_j(U_i)$ and returns a sample $s_i \in V$ with probability $D_j(s_i)/D_j(V)$.  
\begin{definition}
    Ratio Oracle:   The ratio query $Ratio_j(A_v)$ 
    \begin{enumerate}
        \item picks an element $e$ in $O_i \cup \{U_i\}$ (elements of $O_i$ and the set $\{U_i\}$ itself) with probability $\frac{D_j(e)}{D_j(O_v \cup U_v)}$. If $e = \{U_i\}$ then
       \begin{enumerate}
        \item An atom $V \in At(U_i)$ is picked with probability $\frac{|V|}{|U_i|}$.
        \item The sample $s_i$ is generated by the $COND_j(V)$. 
    \end{enumerate}
    \end{enumerate}
  %  , and if $e = \{U_i\}$ then it picks an atom $V$ in $At(U_i)$ with probability $|V|/|A_i$ and returns a sample $s_i \in V$ with probability $D_j(s_i)/D_j(V)$.  
\end{definition}



We are interested in the behavior of the tester $T$ that uses the same function $f_T$  to determine the next query (that is, they have the same decision tree $R$) but  is provided samples from the ratio oracle  instead of the actual $COND$  oracle. %(note that the distribution over the outcomes now changes but the tester still uses the same  function $f_R$ (decision tree $R$) to determine the next node given an outcome). 
Though, ratio query $Ratio_j(A_v)$  also depends on input distributions  but in a less complicated manner. This is because the randomness in sampling atoms from $U_v$ is now independent of input distributions. That is, now this randomness can be seen as the internal randomness of the tester. The tester now can be as some distribution over deterministic counterpart of\footnote{Note that we are already considering deterministic counterpart of core adaptive testers. What we mean here is the deterministic counterpart of the tester which itself is the deterministic counterpart of core adaptive testers} testers obtained by fixing the internal randomness (in each possible ways). The crucial aspect is that each of these deterministic counterparts  now only has $q^q$ nodes (because at most $q$ choices are available at every step). Now the threshold value of $q$ can be chosen $\Tilde{\Omega(\log \log n)}$ so that every node in these deterministic counterparts are good node. Finally, by upper bounding the total variation distance between the distributions for Ratio and $COND$ oracles, we prove that the original tester also will not pass through bad nodes. The notion of good and bad nodes is formalized in the definition~\ref{def:good node}. %However, before we formalize, we define an integer $\phi_A$ associated with any atom $A$.

We first provide intuition for all of the  three conditions. In any atom $A \in At(R)$, the expected number of support from bucket $j$ is $\frac{|A|b \rho^j}{n}$. We would like that the actual number is concentrated tightly around its expectation for all atoms  and for all buckets $j \in [r]$. This  happens if this expectation value is either too large or too small than one. The first condition exactly characterizes this.  Next, we want that an atom either intersects with a large number of buckets  (at least $\phi$, such atoms are called \emph{large} atoms) or does not intersect with any bucket (such atoms are called \emph{small} atoms). The second condition (together with the concentration condition in the first) exactly characterizes it. This condition will be necessary when we will prove that with high probability, no two samples can be from the same bucket. To explain the third condition, we define $\phi_A$ associated with each atom $A$.

\begin{definition}
    For any atom $A \in At(R)$,   $\phi_A$ is minimum  integer $\triangle \in \{0,1,\dots,r-1\}$ such that  $\frac{|A|b \rho^{r-\triangle}}{n} < 1/\alpha$ and if such an integer does not exist then $\phi_A =r$. In other words, $\phi_A$ is the number of buckets with which $A$ has a large intersection.  %is an unique integer in $[r - \frac{\log (\frac{ n}{|A|b })}{\log \rho}+\frac{\log \alpha}{\log \rho},r+1  - \frac{\log (\frac{ n}{|A|b })}{\log \rho}-\frac{\log \alpha}{\log \rho}]$.
\end{definition}


To explain the third condition, we would like that the probability mass of $U_v$ is too heavy or too light with respect to the probability mass of any single element. Note that if $U_v$ has non-zero mass then the expected probability mass of $U_v$ is $\frac{\sum_{A \in At(U_v)} \phi_A |A|}{rn}$. %We want this expected value to be incomparable to probability mass of any single element.
%Note that $\frac{\log \alpha}{\log \rho} = O(\frac{\log \log n}{\sqrt{\log n}}$. Therefore, $\phi_A$ is a unique integer value in $[r - \frac{\log (\frac{ n}{|A|b })}{\log \rho}+\frac{\log \alpha}{\log \rho},r+1  - \frac{\log (\frac{ n}{|A|b })}{\log \rho}-\frac{\log \alpha}{\log \rho}]$. Intuitively, for any large atom $A$,  $\phi_A$ is the number of buckets that have a large intersection with atom $A$. By definition of large atom, we have $\phi_A \ge \phi$ for all large atom $A$.
%Informally, to analyze the ratio tester, it suffices to analyze the deterministic variant (by Yao's minmax theorem) in which these internal randomnesses are fixed (in an arbitrary way). 
%This then reduces the size of the decision tree from $2^{O(q^2)}$ to $2^{q \log q}$, which allows us to show that $\Tilde{\Omega}(\log \log n)$ queries are  needed to distinguish between YES and NO instances (from earlier $\Omega(\sqrt{\log \log n})$). Finally, we will show that the behavior of the ratio tester and the actual tester does not change much thereby allowing us to show the same lower bound for the actual tester.



%First, we want to highlight that the main analytic difficulty of the problem lies in the fact that the distribution $COND_(A_u)$ can not be explicitly (or in closed form) described as a function of $x$ (obviously, it is fully characterized by $x$ via the distribution $D_x$).   The ratio distribution, on the other hand, has a simpler description as a function of $x$ as the second step, i.e., sampling from the atoms of $U_i$ is independent of $x$ (the first step is the same as that of actual distribution and hence ratio distribution overall depends on $x$). It would be nice if we show that the behavior of $T$ does not change much even if $T$ is provided samples from ratio distribution. If this is true, then it suffices us to show lower bound when $T$ is provided samples from ratio distribution at every step (which should be relatively easier). In fact we will show that the total variation distance between the ratio and the actual distribution is small and hence replacing actual distribution by ratio distribution does not much change the error probability.

%though ratio distribution depends on $x$ (via $D_x$) only on the first step
\iffalse
We will show the following theorems. We fix $q \le \frac{\log \log n}{100 \log \log \log n}$.
\begin{theorem}
    \label{thm:lower-bound-tester(ratio)}
Suppose $x$ and the distribution $D_1$ and $D_2$ is randomly constructed as before. Any tester that distinguishes YES and NO instance correctly with high probability, when given access to ratio distribution of $D_1$ and $D_2$, must have error probability $p_r \ge 3/4$.
\end{theorem}

\begin{theorem}
    \label{thm:lb-ratio-implies-actual}
Suppose $x$ and the distribution $D_1$ and $D_2$ is randomly constructed as before. The error probability of a tester (when given original distribution), must have error probability $p_a \ge p_r - o(1) \ge 3/4 - o(1)$.
\end{theorem}
\fi


Throughout the paper, we have $\gamma = (\log \log n)^{9}, \alpha = (\log n)^{(\log \log n)^2}$.
\begin{definition}
\label{def:good node}
    A node $v$ of the decision tree $R$ (recall that $\bm{A}_v = (A_{v_0},\dots,A_{v_i})$) is called good for $x$ if it satisfies all of the following conditions (recall that $b =2^x)$:
    \begin{enumerate}
        \item For any atom $A \in At(\bm{A}_v)$, we have for all bucket $j \in [r]$, either $ \frac{|A|b\rho^j}{n} \ge \alpha$ or $\frac{|A|b\rho^j}{n} \le \frac{1}{\alpha}$. %If the former condition holds, we say atom $A$ is large, and if the later condition holds we say $A$ is small,
        \item For any atom $A \in At(\bm{A}_v)$, we have either $\frac{|A|b \rho^{r-\phi}}{n} \ge \alpha$ or $\frac{|A|b \rho^{r}}{n} \le 1/\alpha$. If the former condition holds, we say atom $A$ is large, and if the latter condition holds we say $A$ is small,
        \item For all $U_{v_j}$ ($j \le i$), we have either $\frac{\sum_{A \in At(U_{v_j})} \phi_A |A|}{rn} \ge \gamma$ or $\frac{\sum_{A \in At(U_{v_j})} \phi_A |A|}{rn} \le 1/\gamma$.
    \end{enumerate}
     A node $v$ is called bad for $x$ if it is not good for $x$.
\end{definition}

%An $i$ configuration is called bad if it is not good. 
Note that for any small atom $A$, we have $\phi_A = 0$ and for any large atom $A$, we have $\phi_A \ge \phi$.  
Also given $x$, whether a given node $v$ is good or bad  depends only  on the size of each atom in $At(\bm{A}_v)$. Also, if a node is bad then all its descendants are also bad.
\begin{lemma}~\cite{}
\label{lem:prob-x-bad-u}
     The probability that node $v$ of $R$ is bad is at most $\frac{2^q (\phi \log \rho + r \log \alpha + r \log \gamma)}{\log n} \le  \frac{2^q (\log \log n)^5}{\sqrt{\log n}}$. Therefore, the probability that all nodes of $R$  are good is at least $1- \frac{|R|2^{q} (\log \log n)^5 }{\sqrt{\log n}} \ge 1 - o(1)$ if $q \le \frac{\sqrt{\log \log n}}{10}$.
\end{lemma}


\begin{lemma}~\cite{}
\label{lem:if-good-then-lb}
     Conditioned on the event that all nodes in $R$ are good, if $q = poly(\log \log n)$ then the tester can not correctly classify the YES and NO instances with high probability. 
\end{lemma}
 The above two lemmas directly gives a lower bound of $\Omega(\sqrt{\log \log n})$.
We want to emphasize few points here. % Note that, by definition, whether  $x$ is good or bad for a node $u$ depends only on size of each atom in $At(A_1,\dots,A_i)$. Given $K$ nodes, in a straightforward way, probability that $x$ is good for all $K$ nodes of $R$ is at least $1- \frac{K 2^q (\phi \log \rho + r \log \alpha + r \log \gamma)}{\log n}$. 
  The barrier of $\Omega(\sqrt{\log \log n})$ comes from the  Lemma~\ref{lem:prob-x-bad-u}, the lower bound in Lemma~\ref{lem:if-good-then-lb} holds even when\footnote{In \cite{}, in theorem statement, $q$ is stated as $\sqrt{\log \log n}$ as perhaps there is no incentive to prove for larger value of $q$ since the first part already restrict the value of $q$.} $q = poly(\log \log n)$. Finally, for the second part, it suffices to condition on the event that the tester does not pass through a bad node with high probability (which obviously holds if all nodes in $R$ are bad with high probability). We rephrase the above lemma for our purpose and give our own proof in appendix.
\begin{lemma}
\label{lem:if-good-then-lb-rephrased}
     Conditioned on the event that the tester does not pass through bad nodes, even if $q = poly(\log \log n)$ then the tester can not correctly classify the YES and NO instances with high probability. 
\end{lemma}
%recall that we wanted no two samples to fall on same bucket because we want first step to just depend on the index of the bucket where the samples belong. However, recall that first step involve sampling from $O_i \cap \{U_i\}$. We also want that the probability mass of $U_i$ is incomparable to each samples obtained so far. This will be of course true if the expected probability mass of $U_i$ which is $\frac{\sum_{A \in At(U_i)} \phi_A |A|}{rn}$ is either too heavy or too less that the probability mass of a single element in each bucket. Since no two samples are from the same bucket and probability mass of an element in each bucket differs exponentially, there will exist a total order on $O_i \cup \{U_i\}$ and given this total order, the first step will pick the heavies one.



%Given a set of $K$ $i$-configurations (think of the set of all possible configurations for a tester), we say $x$ is bad (good) for all $K$ collections if $x$ is bad for some (good for all) $i$-configuration. 
%Note that given $x$, whether a given $i$-configuration is good or bad only depends on the size of each atom in $At(A_1,\dots, A_i)$. If an $i$-configuration is bad for $x$ then either $\frac{n}{|A|\rho^j \alpha} < 2^x < \frac{n\alpha}{|A|\rho^j}$ for some $j \in [r]$ or $\frac{n}{|A|\rho^{r}} < 2^x  < \frac{n \rho^{\phi}}{|A|\rho^{r}}$ or $1/\gamma \le \frac{\sum_{A \in At(U_i)} \phi_A |A|}{rn} \le \gamma$. We are interested in the upper bound on the values of $x$ for which the set of $K$ $i$-configurations is bad. For the same, we can sum the number values of $x$ which will satisfy each of the three inequalities, for each atom $A$ and $U_i$ in the configuration, for each of the possible $K$ configurations.  For instance, the first inequality can be satisfied by at most $\log (\alpha^2)$ values of $x$ for  a given atom, and since the total number of possible atoms in a set of $K$ $i$-configurations is at most $K 2^q$, the inequality rules out at most $2K 2^q \log \alpha$ values of $x$. Rephrasing the lemma of ~\cite{},
\iffalse
\begin{lemma}
   Total at most $K. 2^q (\phi \log \rho + r \log \alpha + r \log \gamma)$ values of $x$ can be bad for a set of $K$ configurations,. In other words,  when $x$ is chosen at uniformly at random, the probability that $x$ is good for all $K$ configurations is at least $1- \frac{K 2^q (\phi \log \rho + r \log \alpha + r \log \gamma)}{\log n}$.
\end{lemma}
We want to point out that the above lemma in ~\cite{} was shown for a set of all possible configurations of the tester. But in a straightforward way, it holds for any set of configurations as stated in the above lemma. Then they show the following lower bound.

\begin{lemma}
     Assuming that the tester does not reach a bad configuration, the distribution over leaves are close by for both YES and NO instances for $q = poly(\log \log n)$\footnote{In \cite{}, since $q$ has to be $\sqrt{\log \log n}$ so they were not interested if this lemma is valid for $q = poly(\log \log n)$ or not.}.
\end{lemma}


Note that for a tester, the total number of possible configurations is $K = 2^{q^2}$. When $q = o(\sqrt{\log \log n})$ then we have $K. 2^q (\phi \log \rho + r \log \alpha + r \log \gamma) = o(\log n)$ and hence with $1-o(1)$ probability, the tester never reaches a bad configuration. Note that if $q \ge \sqrt{\log \log n}$ then with high probability, the tester can reach a bad configuration and hence their analysis is tight, i.e., it can not provide a better lower bound that $\sqrt{\log \log n}$. Finally, they show that conditioned on the event that the tester never reaches a bad configuration, a tester can not distinguish YES or NO instance if it makes $q = o(\sqrt{\log \log n})$ queries. Note that the behaviour of the tester differs in YES and NO instance because the distribution over outcomes (via $COND(O_i \cup U_i)$ query) differs in YES and NO instance. In `\cite{}, it is shown that in both these YES and NO instances, though the distribution of outcome differs but not by much (given that the tester is not in bad configuration, which can be assumed) and hence both instances induces close by (in total variation distance) distributions on the leaves of the decision tree if $q = o(\sqrt{\log \log n})$. 
%Ideally, we would like that in any atom $a$
\fi
%\subsection*{Our Proof}
%We will first prove the following Theorem and, which are the heart of our lower bound proof.   
Again, we want to remind that if $q = \frac{\log \log n}{100 \log \log \log n}$ then the size of the decision tree $|R|$ is $2^{q^2} = O((\log n)^{\log \log n})$ and hence  Lemma ~\ref{lem:prob-x-bad-u} will not imply the following theorem.%it is not possible to prove that all nodes in $R$ are good with high probability (similar.

\begin{theorem}
    If $q \le \frac{\log \log n}{100 \log \log \log n}$   then with high probability, the tester $T$ when provided samples from the ratio oracle, does not pass through bad nodes.
\end{theorem}
\begin{proof}
   % Such a tester at any step $i$,  samples an element $e$ in $O_i \cup \{U_i\}$ with probability $D_j(e)/D_j(U_i)$, and if $\{U_i\}$ is sampled then it picks an atom $V \in At(U_i)$ with probability $|V|/\|U_i|$, and then samples $s_i$ in $V$ with probability $D_j(s_i)/D_(V)$. 
    
    Note that the tester can itself simulates step 1(a) of the ratio oracle,  as it involves picking an atom $V \in At(U_i)$ with probability $|V|/\|U_i|$ (which is independent of the input distributions). Fixing these internal randomnesses in advance, in all possible ways, gives  several deterministic counterparts of testers say $T_1,\dots, T_w$ for some $w \ge 1$ and the original tester can thus be seen as some probability distribution say $(p(T_1),\dots,p(T_m))$ over testers $T_1,\dots,T_w$. Note that each $T_j$ has at most $q^q$ nodes (because the number of children of any node $v$ can be at most $q$, namely (at most $q$) elements in $O_v \cup \{U_v\}$). %The original tester can be seen as some probability distribution say $(p(T_1),\dots,p(T_m))$ over testers $T_1,\dots,T_m$. 
    If $q \le \frac{\log \log n}{100 \log \log \log n}$  then by Lemma~\ref{lem:prob-x-bad-u},   for any fixed $T_j$ ($j \le w$), with probability at least $1 - o(1)$,  each node of $T_j$ is good.
    \begin{align*}
        \Pr[T \text{ reaches a bad node} ]& = \frac{\sum_{x \in \mathcal{X}} \Pr[T \text{reaches a bad node}| x ]}{|\mathcal{X}|}\\
        & = \frac{\sum_{x \in \mathcal{X}}  \sum_{j=1}^{m} p(T_j)   \Pr[T_j \text{reaches a bad node}| x ]}{|\mathcal{X}|}\\
        &= \frac{\sum_{j=1}^{m} p(T_j)  \sum_{x \in \mathcal{X}}    \Pr[T_j \text{reaches a bad node}| x ]}{|\mathcal{X}|}\\
        & = \sum_{j=1}^{m} p(T_j)  \Pr[T_j \text{reaches a bad node}] \\
        & = o(1)
      \end{align*}
\end{proof}
Interestingly, using the above theorem, we  will show that the original tester (tester when provided samples from $COND$ oracle)  also does not pass through bad nodes with high probability. Before that, we note that all good nodes will have a tight concentration (recall the definition ).
\


\begin{lemma}
\label{lem:conc-size-atom}
    With  probability at least $1 - \frac{1}{poly(\log \log n)}$, for all atoms $A \in \bm{A}_v$ for any good node $v$, we have:
    
       % \item If an atom $A \in At(\bm{A}_v)$ is small then we have $D_1(A) = D_2(A) =0$.
        %\item If an atom $A \in At(\bm{A}_v)$ is large then 
        \begin{enumerate}
            \item for all $j \ge  r - \phi_A +1$,   $|B_j \cap A| \in [1-\frac{1}{\gamma}, 1+ \frac{1}{\gamma}] \frac{|A|b \rho^j}{n}. $ Moreover, both  $|B^e_j \cap A|, |B^f_j \cap A| \in [1-\frac{1}{\gamma}, 1+ \frac{1}{\gamma}] \frac{|A|b \rho^j}{2n}$
            \item for all $j \le r - \phi_A$, $|B_j \cap A| = 0$.
        \end{enumerate}            
  
\end{lemma}
\begin{proof}
    If  $\frac{|A|b\rho^j}{n} \le \frac{1}{\alpha}$ for any atom $A$ and $j \in [r]$ then by Markov's inequality $\Pr[|A \cap B_j| > 0] \le \frac{1}{\alpha}$.  Taking union bound over all good atoms (which can be at most $2^{q^2} \le (\log n)^{\log \log n}$) and all $j \in [r]$, with probability at least $1 - \frac{1}{poly(\log \log n)}$, for any atom $A$ and $j \le r - \phi_A$, we have $|B_j \cap A| = 0$.


    Note that $\E[|B^e_j \cap A|] = \frac{|A|b \rho^j}{2n} \ge \alpha/2$ for $j \ge r - \phi_A +1$. Therefore,  $\Pr[|A \cap B^e_j| \not \in [1-\frac{1}{\gamma}, 1+ \frac{1}{\gamma}] \frac{|A|b \rho^j}{2n}] \le O(exp(-\alpha/\gamma^2))$. Similarly, $\Pr[|A \cap B^f_j| \not \in [1-\frac{1}{\gamma}, 1+ \frac{1}{\gamma}] \frac{|A|b \rho^j}{2n}] \le O(exp(-\alpha/\gamma^2))$. Hence $\Pr[|A \cap B_j| \not \in [1-\frac{1}{\gamma}, 1+ \frac{1}{\gamma}] \frac{|A|b \rho^j}{n}] \le O(exp(-\alpha/\gamma^2))$.
\end{proof}
\begin{corollary}
   With  probability at least $1 - \frac{1}{poly(\log \log n)}$, for all good nodes $v$ and for all  atoms $A \in At(\bm{A}_v)$, we have $D_1(A),D_2(A) \in [1-1/\gamma,1+1/\gamma] \frac{\phi_A |A|}{rn}$. Therefore, for any query set $U_{v_j}$ ($j \le i$), we have $D_1(U_{v_j}),D_2(U_{v_j}) \in [1-1/\gamma,1+1/\gamma] \frac{\sum_{A \in At(U_{v_j})} \phi_A |A|}{rn}$.
\end{corollary}
\begin{proof}
    $D_j(A) = \sum_{j} \frac{|A \cap B_j|}{br \rho^j} \in  [1-\frac{1}{\gamma}, 1+ \frac{1}{\gamma}] \sum_{j:\ge r - \phi_A +1} \frac{|A \cap B_j|}{br \rho^j} = [1-\frac{1}{\gamma}, 1+ \frac{1}{\gamma}]\frac{\phi_A |A|}{rn}$. It immediately follows that $D_j(U_{v_j}) \in [1-1/\gamma,1+1/\gamma] \frac{\sum_{A \in At(U_{v_j})} \phi_A |A|}{rn}$
\end{proof}
\begin{theorem}
    If $q \le \frac{\log \log n}{100 \log \log \log n}$  then with high probability, the tester (when provided samples via actual $COND$- model)   does not reach a bad node.
\end{theorem}
\begin{proof}
%Let $p_r(i)$ and $p_a(i)$  denotes the probability the the tester when given ratio distribution and the actual distribution respectively, reaches some bad node till depth $i$. 

%Note that the ratio oracle and the $COND$ oracle differs only in step 1(a). 

For notation, we use $T(ratio)$ and $T(cond)$ for testers with decision tree $R$ and samples provided by ratio and $COND$ oracles respectively. Let $E$ be the event mentioned in the statement of the  Lemma . We will upper bound the total variation distance between the distribution over nodes of $R$ at any depth $i \le q$, denoted by $tv(i)$, for $T(ratio)$ and $T(COND)$, conditioned on event $E$. Then, the overall total variation distance can be at most $\Pr[\overline{E}]$ plus the total variation distance conditioned on $E$.

   Note that if a node is bad then its all descendants are also bad. Let $R'$ be the subtree of $R$ where any bad node is removed if there exists an ancestor of this node which is also bad. Note that in $R'$, all bad nodes are leaves. Note that the probability of reaching a bad node in $R$ is the same as that in $R'$. %Let $D_R(i)$ and $D_C(i)$ be the distribution on nodes of $R'$ at depth $i$ for a tester provided with ratio and $COND$ oracle respectively. Our induction hypothesis is that $||D_R(i) - D_C(i)||_{TV} \le \frac{i}{\gamma}$. This is trivially true for $i=1$. Now we will show that $||D_R(i+1) - D_C(i+1)||_{TV} \le \frac{i+1}{\gamma}$.
%Let $d(i)$ be t

Consider any good node $v$ at depth $i$. We will upper bound the total variation distance between distributions over children of $v$  for the $T(ratio)$ and $T(COND)$ (conditioned on the fact that the tester is currently at $v$). If this upper bound is $\epsilon$ then we have $tv(i+1) \le tv(i) + \epsilon$. Note that $T(ratio)$ and $T(cond)$ only differs in step 1(a) so it suffices to upper bound the distance for distribution over atoms of $U_v$. If $U_v$ has no large atom then we have $D_1(U_v) = D_2(U_v) = 0$ (we conditioning on event $E$). In this case, total variation distance is zero. So let us assume that $U_v$ has at least one large atom. Let $V_m$ be the atom of the largest size in $U$. Hence, $\phi_{V_m} \ge \phi$.
%If $U_u$ has no large atom then we have $D_1(U_u) = D_2(U_u) = 0$ (we conditioning on event $E$). In this case, ratio and $COND$ oracle are same. So let us assume the $U_u$ has at least one large atom. Let $V_m$ be the atom of the largest size in $U$. We will upper bound the total variation distance between the distribution over atoms of $U_u$ for tester when provided ratio and conditional sampling respectively.
Further, as we are conditioning on $E$, for all $j \in \{1,2\}$, we hace  $D_j(V) = \theta^j_V \frac{\phi_V |V|}{\sum_{W \in At(U)} \phi_W |W|}$ where $\theta^j_V \in [1-1/\gamma,1+1/\gamma] $. Now the total variation distance is given by:
%We first note that if $U$ is a small atom
%Consider a distribution over atoms of $U$, where every atom $V \in At(U)$ is picked with probability $\frac{|V|}{|U|}$. Consider another distribution over atoms of $U$ say $D_U$ in which every atom $V \in At(U)$ is picked with a probability that lies in $\theta_V \frac{\phi_V |V|}{\sum_{W \in At(U)} \phi_W |W|}$ where $\theta_V \in [1-1/\gamma,1+1/\gamma] $. We want to upper bound the total variation distance between these distributions. Let $V_m$ be the largest atom in $U$. The total variation distance between these two distribution is given by: 


%If the tester does not reach a bad configuration then we have with  probability at least $1 - \frac{1}{(\log n)^{(\log \log n)^5}}$, for all $V$, $D(V) = \theta_V \E[D(V)] = \theta_V \phi_V \frac{|V|}{rn}$ where $\theta_V \in [1-1/\gamma,1+1/\gamma]$.


%Then at any step $j \le i$, for any distribution, 
\begin{align*}
  &  \sum_{V \in At(U)}| \frac{\theta_V \phi_V |V|}{\sum_{W \in At(U)} \phi_W |W|} - \frac{|V|}{|U|}|\\
    &  = \sum_{V \in At(U): |V| < \frac{V_m}{\rho}}|\frac{\theta_V \phi_V |V|}{\sum_{W \in At(U)} \phi_W |W|} - \frac{|V|}{|U|}| +  \sum_{V \in At(U): |V| \ge \frac{V_m}{\rho}}|\frac{\theta_V \phi_V |V|}{\sum_{W \in At(U)} \phi_W |W|} - \frac{|V|}{|U|}|
\end{align*}
We note that for any $V$ such that $|V| < \frac{V_m}{\rho}$,  both $\frac{\phi_V |V|}{\sum_{W \in At(U_j)} \phi_W |W|}$ and $\frac{|V|}{|U_j|}$ are in $[0,\frac{1}{\rho}]$. Since any $U$ can have at most $2^q \le \log n$ atoms so we have $\sum_{V \in At(U_j): |V| < \frac{V_m}{\rho}}|\frac{\theta_V \phi_V |V|}{\sum_{W \in At(U_j)} \phi_W |W|} - \frac{|V|}{|U_j|}| \le \frac{(1+1/\gamma)\log n}{\rho}$. Further, for any $V,W$ such that $\frac{|V_m|}{\rho} \le |V|,|W| \le |V_m|$, we have $|\phi_V - \phi_W| \in \{0,1\}$. Therefore, $\frac{\phi_{V_m} -1}{\phi_{V_m}} \frac{|V|}{|U|} \le  \frac{\phi_V |V|}{\sum_{W \in At(U_j)} \phi_W |W|} \le \frac{\phi_{V_m} }{\phi_{V_m} -1} \frac{|V|}{|U|}$ and hence  $|\frac{\theta_V\phi_V |V|}{\sum_{W \in At(U)} \phi_W |W|} - \frac{|V|}{|U_j|}| \le (\frac{1}{\gamma} + \frac{1}{\phi_{V_m}}) \frac{|V|}{|U|} \le \frac{2}{\gamma}\frac{|V|}{|U|}$ (as we have $\phi_{V_m} \ge \phi$ since $V_m$ has to be large atom). So the total variation distance is bounded above by $\frac{\log n}{\rho} + \frac{2}{\gamma} \le  \frac{3}{\gamma}$.

Therefore, we have $tv(i+1) \le tv(i) + 3/\gamma$ and so $tv(i) \le  3i/\gamma$ for all $i \le q$.  Overall, the probability of reaching a bad node in $T(cond)$ is at most $\sum_{i=1}^{q} 3i/\gamma + \Pr[\overline{E}] \le q^2/\gamma + \frac{1}{(\log n)^{\log \log n}}$.

%Therefore, the total variation distance on nodes at depth $i+1$ is at most $3/\gamma$ plus the the total variation distance on nodes at depth $i$. This implies that the  total variation distance on nodes at depth $i$ is at most $3i/\gamma$. Therefore, the probability of reaching a bad node at any depth $i$ in $T(ratio)$ is at most $3i/\gamma$ plus the probability of reaching a bad node at any depth $i$ in $T(cond)$. Overall, the probability of reaching a bad node in $T(cond)$ is $\sum_{i=1}^{q} 3i/\gamma + \Pr[\overline{E}] \le q^2/\gamma + \frac{1}{(\log n)^{\log \log n}}$.

%If $T(ratio)$ can reach bad nodes with probability at most $p_r$ then actual tester can reach bad nodes with probability at most $p_r + 3q/\gamma + \frac{1}{(\log n)^{(\log \log n)^5}}$. 

%Since for any $V$, we have $D(V) \in  [1 - 1/\gamma, 1+ 1/\gamma] \phi_V \frac{|V|}{rn}$ therefore $\sum_{V \in At(U_j)}|\frac{D(V)}{D(U_j)} - \frac{|V|}{|U_j|}| \le $

%Therefore, $p_a(i+1) \le p_a(i) + $

%The only difference is in sampling atoms from $U_i$. The ratio distribution picks an atom $V \in At(U_i)$ with probability $\frac{|V|}{|U_i|}$ whereas the actual distribution picks an atom $V$ with 
\end{proof}
The above theorem together with Lemma 2 directly proves the following theorem. For completeness, we provide the complete proof in appendix.
\begin{theorem}
    If $q \le \frac{\log \log n}{100 \log \log \log n}$ then the total variation distance on distribution over leaves for both YES and NO instances is $o(1)$. Hence, a tester with $q \le \frac{\log \log n}{100 \log \log \log n}$ must have large error probability to distinguish YES and NO instance.
\end{theorem}


==> abstract.tex <==
\begin{abstract}
    We study the equivalence testing problem where the goal is to determine if the given two unknown distributions on $[n]$ are equal or $\epsilon$-far in the total variation distance in the conditional sampling model (CFGM, SICOMP16; CRS, SICOMP15)  wherein a tester can get a sample from the distribution conditioned on any subset. Equivalence testing is a central  problem in distribution testing, and there has been a plethora of work on this topic in various sampling models.
    
   Despite significant efforts over the years, there remains a gap in the current best-known upper bound of $\Tilde{O}(\log \log n)$ and lower bound of $\Omega(\sqrt{\log \log n})$.
   Closing this gap has been repeatedly posed as an open problem (listed as problems 66 and 87 at sublinear.info). In this paper, we completely resolve the query complexity of this problem by showing a lower bound of $\Tilde{\Omega}(\log \log n)$. To this end, we develop a novel and generic proof technique that enables us to break the $\sqrt{\log \log n}$ barrier for several other problems in distribution testing such as label-invariant properties. 
\end{abstract}

==> temp.tex <==
\section{Simple Adaptive Testers}
\begin{definition}
    ($i$-configuration of simple testers): Given a sequence of query $(O_1 \cup U_1,\dots,O_i \cup A_i)$ and samples $\boldsymbol{s}_i = (s_1,\dots,s_i)$, a $i$-configuration of a simple tester consists of $\log i + 1$ bits, indicating  whether
    \begin{enumerate}
        \item $s_i$ is fresh or already seen (i.e., $s_i = s_k$ for any $k < i$ or not. This takes only one bit).
        \item If $s_i$ is not fresh then any $1 \le k <i$ such that $s_i = s_k$ (This takes $\log i$ bits).
    \end{enumerate}
\end{definition}
Note that the $1$-configuration,\dots,$q$-configuration together contain all  information about collisions that have happened among $\boldsymbol{s}$.

\begin{definition}
    (simple-adaptive testers): A simple adaptive tester for a pair of distributions is an algorithm $T^s$ that 
    \begin{enumerate}
        \item In the $i$-th phase, based only on its own internal randomness and the configuration of the previous queries $A_1,\dots,A_{i-1}$ and samples obtained $(s_1,\dots,s_{i-1})$ (whose labels it does not know), $T$ provides:
        \begin{enumerate}
            \item  a set $U_i \in [n] \setminus  \{s_1,\dots,s_{i-1}\}$ (a set  consisting of  only fresh, not already seen elements).
            \item set $O_i \subseteq \{1,\dots,i-1\}$ (which of the samples $s_1,\dots,s_{i-1}$   will be included in the next query. The labels of these samples are unknown, but are indexed by the index of the query which returned them).

            Based on these specifications, the next query $A_i$ is set as:
            \begin{align}
                A_i = O_i \cup U_i
            \end{align}
        \end{enumerate}
        \item fixes a number $j \in \{1,2\}$ (fixes the distribution $D_1$ or $D_2$ on which $T$ will perform the conditional query)
        \item sample $\bar{s}_i \in COND_{D_j}(O_i \cup \{U_i\})$ is drawn. If $\Bar{s}_i \in O_i$ then $s_i := \bar{s}_i$ (but $s_i$ is  not revealed to $T$). If $\Bar{s}_i =\{U_i\}$ then $T$   samples $s_i \in COND_{D_j}(U_i)$ (again  $s_i$ is  not revealed to $T$).  This defines the $i$-configuration of $(A_1,\dots,A_i)$ and $(s_1,\dots,s_i)$ which is revealed to $T$.  Put differently, the algorithm only learns (i) if the sample is fresh or already seen, and (ii) if it is one of the previous samples, in which stage(s),  it has already seen it.
        \end{enumerate}
        After $q = q(\epsilon,n)$ queries, the tester $T$ returns ACCEPT or REJECT based  on information it has, i.e., only on the configuration of $(A_1,\dots,A_q)$ and $(s_1,\dots,s_q)$. 
\end{definition}


%At any step $i$, the tester chooses a set $O_i \subseteq \mcO_{i-1}$ and $U_i \subseteq \mcU_{i-1}$ and perform $COND(O_i \cup U_i)$ query for both distributions. Let $s^i_1 \in [n]$ and $s^i_2 \in [n]$ be the sampled elements of these conditional queries for both distributions respectively. The labels of $s^i_1$ and $s^i_2$ are not revealed to the tester. Instead, the tester will be given information whether $s^i_j = s^{i'}_{j'}$ or  $s^i_j \neq s^{i'}_{j'}$ for any $j, j' \in \{1,2\}$, $i' \le i$.
%Let  $\mathcal{S}_{=}:=\{S_1,\dots,S_k\}$  be the equivalence class on $\mcO_i$  based on equality, i.e., $S_j \subseteq \mcO_i$ and  $s^{i_1}_{j_1} = s^{i_2}_{j_2}$ for all $s^{i_1}_{j_1}, s^{i_2}_{j_2} \in S_j$, for all $j \in [k]$. A simple adaptive tester has full knowledge of $\{S_1,\dots,S_k\}$ at any step $i \le q$.
%define \mcO_i = $\{s^u_v\}_{u \in [i], v \in \{1,2\}}$
%The element $k$ is revealed via the minimum value of $j$ for which $k \in U_j$. 

Note that the $i$th configuration can be described by at most $2 \log i$ bits so the total number of configurations (or nodes in the decision tree) is at most $2^{2q \log q}$.
